Rethinking the Role of Demonstrations: What Makes In-Context Learning Work?

Large language models (LMs) are able to in-context learn -- perform a new task via inference alone by conditioning on a few input-label pairs (demonstrations) and making predictions for new inputs. However, there has been little understanding of how the model learns and which aspects of the demonstrations contribute to end task performance. In this paper, we show that ground truth demonstrations are in fact not required -- randomly replacing labels in the demonstrations barely hurts performance on a range of classification and multi-choce tasks, consistently over 12 different models including GPT-3. Instead, we find that other aspects of the demonstrations are the key drivers of end task performance, including the fact that they provide a few examples of (1) the label space, (2) the distribution of the input text, and (3) the overall format of the sequence. Together, our analysis provides a new way of understanding how and why in-context learning works, while opening up new questions about how much can be learned from large language models through inference alone.

==> sections/01-intro.tex <==
Large language models (LMs) are capable of {\em in-context learning}---they can perform a new task during inference by simply conditioning on a few input-label pairs (called {\em \demo})~\citep{brown2020language}. % to make a prediction to the test input.
%Prior work has suggested that the model {\em ``learns''} a new task from these input-label pairs as humans do~\citep{brown2020language,zhao2021calibrate,liu2021makes}.
In-context learning outperforming zero-shot inference on a wide range of tasks~\citep{zhao2021calibrate,liu2021makes} clearly shows the value of \demo.
However, there is little understanding of {\em how} this learning works and {\em which} aspects of the \demo\ contribute to end task performance.

%which tasks

%Although such learning seemingly uses to input, output pairings 

%The demonstrations  example inputs, example outputs, and examples of  

%provide many different types of signals for learning, they 

%input space, output space, and a few examples of input, output pairs


%Although this in-context inference works well in practice, often outperforming zero-shot and other learning methods, 


%and whether the model recovers the correlation between inputs and outputs for the new task {\em from} the \demo.

%the model learns from the \demo\ given that it is only given at inference, and whether the model recovers the correlation between inputs and outputs for the new task {\em from} the \demo.
%the \demo\ is actually effective to inform the model of the correlation between inputs and outputs for a new task.
%This implies the correlation between inputs and labels in the demonstration is key to in-context learning, informing the model of the semantics of the new task.

\begin{figure}[t]
\centering \footnotesize
\resizebox{\columnwidth}{!}{\includegraphics[trim={4cm 0.6cm 4cm 1cm},clip]{figures/intro_cls.pdf}}
\resizebox{\columnwidth}{!}{\includegraphics[trim={4cm 0.6cm 4cm 1cm},clip]{figures/intro_mc.pdf}}
\vspace{-.1em}
\caption{
    Results in classification (top) and multi-choice tasks (bottom), using LMs with 774M, 6B, and 175B parameters, respectively.
    %(all with channel).
    \ari{most people won't know what "with channel" means here until they read the rest of the paper, and it's not really important for the immediate point. I would just include a reference to the experimental section that describes the details instead of trying to fill them in here. Probably the same for the next sentence, sinc e you want to get to  the last sentence as quickly as possible.}
    \sewon{I think some people might still want to see some clarification about the experiment.. I squeezed details into one sentence---is it better?}
    Reported on six datasets on which GPT-3 is evaluated; the channel approach is used;
    see Section~\ref{sec:main} for the full details.
    %Reported on six datasets on which GPT-3 is evaluated; full results on 6 datasets for other models are in Figure~\ref{fig:main-results}.
    In-context learning performance drops only marginally when labels in the \demo\ are replaced by random labels.
    %\ari{ideally, you want this graphic to make sense before someone reads the caption. therefore, I recommend the labels "No Demo", "Gold Labels", and "Random Labels"—it's slightly less specific, but just saying "random" without a noun is too confusing and ruins the "instant communication" factor.}
    %\ari{just leaving a little note here that the diagram should eventually label the top and bottom parts of the figure visually not just in the caption.}
}\label{fig:intro}
\end{figure}

In this paper, we show that the groundtruth input-label mapping \ari{I know we've all struggled to come-up with a good phrase, but I don't think ``input-label mapping'' suffices, I really don't think most people will get it. We might want to make a macro for this so we can change it later.} in the \demo\ is much less important than previously thought (Section~\ref{sec:main}).  \ari{we really need a diagram to show these different options—just relying on our accurate technical descriptions won't be sufficient for giving people who don't do ICL all the time good intuition.}
In fact,
replacing labels with random labels
%randomly replacing the labels
in the \demo\ barely hurts performance (Figure~\ref{fig:intro}).
%Model performance only drops marginally when randomly replacing the labels in the \demo\ (Figure~\ref{fig:intro}).
%that the input-label correlation in the \demo\ in fact matter significantly less than previously thought (Section~\ref{sec:main}).
%Model performance drops only marginally when labels in the \demo\ are randomly replaced (Figure~\ref{fig:intro}).
The result is consistent over 12 different models including the GPT-3 family~\citep{radford2019language,min2021metaicl,wang2021gpt,artetxe2021efficient,brown2020language}.
%It, overall, strongly suggests that there must be other aspects of the \demo, beyond the mapping from inputs to outputs, that are allowing the model to perform the task. 
This strongly suggests that the input-label {\em correspondence} required to perform the downstream task is not learned from the \demo.
%\ari{I think the basic rule for talking about "learning" in this paper should be that we basically don't describe what we think the model is doing, but we talk about what it's relying on. So I would rephrase this to be something like "This strongly suggests that the relationship between individual inputs and outputs contributes little to the performance of ICL."}

%This strongly suggests that the mapping between inputs and outputs is not the 

%This results is particularly surprising because we know the model can perform the task, and opens up the question of what other aspects of the demonstration make this possible. 

%This indicates that the \demo\ plays little role in informing the model of the correlation between inputs and outputs.
%This indicates that the model {\em does not learn} the input-label correlation from the given \demo.


Further analysis examines which components of the \demo\ actually contribute to performance gains.
%{\em do} lead to good performance (Section~\ref{sec:abl}).
%To explore this question,
We vary the composition of the \demo\ to isolate different possible aspects: the example inputs, the example labels, and the fact that it consists of the `pairs'. %format expected for the task.
\ari{the word examples here feels very weird. how about "distribution"?} %, all of which can be evaluated separately. 
For instance, replacing all labels with the dummy text ``\texttt{answer}'' keeps the example inputs and the form of the pairs, but removes the example labels and the input-label mapping. 
%we can similarly modify the input examples or mapping in isolation, and again measure their contributions.  
%
%replacing inputs with the random sentences removes the original input examples, but preserves everything else.
%
%order to quantify the impact of (1) the input space, (2) the label space, and (3) the input-label format of the \demo.
%For instance, replacing labels to the text ``\texttt{answer}'' preserves the input space and the format of the \demo, but drops the label space and the input-label correlation; replacing inputs from the training data to the random sentences removes the impact of the input space, but preserves others.
%To explore this question, we vary the composition of the \demo\ in order to quantify the impact of (1) the input space, (2) the label space, and (3) the input-label format of the \demo.
%For instance, replacing labels to the text ``\texttt{answer}'' preserves the input space and the format of the \demo, but drops the label space and the input-label correlation; replacing inputs from the training data to the random sentences removes the impact of the input space, but preserves others.
%
%Overall results indicate that (1) the input space is key for both classification and multi-choice tasks, (2) the output space follows the next\ari{don't know what this means}, and (3) the format of the demonstration matters much in classification but not in multi-choice.
Overall results indicate that (1) input examples and the label examples are both key to in-context learning,
%(2) the input-label `format' in the \demo\ matters much in classification but not in multi-choice,
(2) keeping the form of the `pairs' is significant in the case of classification,
and (3) finetuning with an in-context learning objective~\citep{min2021metaicl} encourages to exploit components that are easier to capture (e.g., the format, rather than the input-label correspondence).
%in classification asks, 56\% of the gains from in-context learning is preserved when we replace labels to the text ``\texttt{answer}'' so that the model knows the domain of the text and the format, but not the label space and the input-label correlation.

%Our findings suggest that it is possible to  achieve competitive performance without any labeled data by leveraging the demonstration. In this context, we propose a strong zero-shot method that forms a silver demonstration using unlabeled data and makes predictions from the LM (Section~\ref{sec:silver}). We show that this method outperforms the previous zero-shot baseline (no demonstration) by 16\%, and achieves nearly $k$-shot performance that uses labeled training data. \ari{As I mentioned in the abstract, I think there is a tension in this paper between "labels don't matter" and "we can generate labels and do almost as good as gold". In order to bridge this gap you have to talk very carefully about "closing the remaining gap" but it's going to be tricky no matter what.}

Together, our analysis provides a new way of understanding the role of the \demo\ in in-context learning (Section~\ref{sec:discuss}).
It suggests that the model does not rely on the groundtruth input-label mapping provided in the \demo,
%unable to recover the groundtruth input-label mapping solely from the \demo \ari{I would definitely not make this claim. I don't think it's clear how we could even test it, since negative results aren't really trusted in NLP. Instead we should talk about what ICL \textit{relies} on},
however, is able to exploit distributions of inputs and labels specified by the \demo, jointly with the input-label correspondence that is likely implicitly learned from the language modeling objective.
%{\em if} the mapping is already implicitly learned from the language modeling objective.
%\ari{I think it will be very tempting to say something like "LMs only know certain tasks and we're just telling them which one this is", but I think we should be very careful not to say that. I think it's a good intuition, but actually, I think it might also be wrong, and I don't think we've really tested that. Indeed, it might be that the tasks we're choosing simply only require some local understanding and hints about the input and output distribution. Instead, I would lean on claims about what parts of ICL appear to actually be important, e.g. the three elements described earlier in the intro. If we include some of the experiments you mentioned (but I don't see here) about changing the labels then \textit{maybe} we could suggest local similarity of the input-output correspondence for the test question is also required, which gets closer to what you're suggesting. But the reality is that we didn't really test what things LMs \textit{can't} do, so we can't make this claim.}
We suggest avenues for future work, including better extraction of the task mapping stored in the LM, making progress on NLP tasks whose mappings are not learned from the LM objective, and an extension of our analysis to instruction-reading models.

%It is very likely that the model exploits its capacities acquired from the language modeling objective when inferring the correlation between inputs and outputs for a downstream task, rather than learning the correlation through the \demo. It is likely that using the \demo\ is only a way to extract that capacity, by specifying the input space, the output space and how they should be formatted.
%This brings up a series of new research questions, such as (1) how to identify capacities of LMs (2) how to extract such capacities for tasks, and (3) how to make progress on tasks that requires capacities that LMs do not have yet.






==> sections/05-abl.tex <==
Section~\ref{sec:main} shows that the groundtruth input-label mapping in the \demo\ has little impact to performance gains from in-context learning.
This section further examines what other components in the \demo\ lead to good performance of in-context learning.

\begin{figure}
\centering \footnotesize
\resizebox{\columnwidth}{!}{\includegraphics[trim={11cm 18.5cm 6cm 2cm},clip]{figures/composition.pdf}}
\caption{
    Four different components in the \demo: the input-label mapping,
    %the example inputs, the example labels and the form of the ``pairs'' (e.g., having the input-label pairs as the {\em form} of the \demo). \ari{This is a great diagram. I think "form of `pairs'" is too confusing as a description though....how about ``paired format''?}
    the label space, the distribution of the input text and the use of input-label pairs.
}\label{fig:composition}
\end{figure}

\definecolor{mygold}{HTML}{fdb462}
\definecolor{myred}{HTML}{fb8072}
\definecolor{mypurple}{HTML}{bebada}
\definecolor{mygreen}{HTML}{8dd3c7}
\newcommand{\goldbox}{\textcolor{mygold}{$\blacksquare$}}
\newcommand{\randombox}{\textcolor{myred}{$\blacksquare$}}
\newcommand{\answerbox}{\textcolor{mypurple}{$\blacksquare$}}
\newcommand{\nolabelbox}{\textcolor{mygreen}{$\blacksquare$}}
\begin{figure*}
\centering \footnotesize
\resizebox{2.1\columnwidth}{!}{\includegraphics[trim={7cm 0.5cm 7cm .5cm},clip]{figures/abl_main_cls_2.pdf}}
\resizebox{2.1\columnwidth}{!}{\includegraphics[trim={7cm 0.5cm 7cm .5cm},clip]{figures/abl_main_mc_2.pdf}}
\caption{
    Results with a series of variants of \demo, in classification (top) and multi-choice tasks (bottom).
    \goldbox$\xrightarrow{}$\randombox\ removes the input-label mapping; \randombox$\xrightarrow{}$\answerbox\ removes the label examples; \answerbox$\xrightarrow{}$\nolabelbox\ removes the form of the pairs;
    hash patterns removes the input examples from the unlabeled training data.
    Discussions in Section~\ref{subsec:abl_result}. \ari{I'm still worried that there's way too much information here and, even at the risk of making the paper 15 pages, we might want to try to expand things out...but that doesn't matter for the Meta submission.}
}\label{fig:abl_result}
\end{figure*}

We identify three components in the \demo\ aside from the input-label mapping:
%(1) the example inputs, (2) the example labels, and (3) the fact that it consists of input-label ``pairs''
(1) the label space, (2) the distribution of the input text, and (3) the use of input-label pairs 
(Figure~\ref{fig:composition}). 
%We hypothesize that components in the \demo\ that potentially lead to performance gains, aside the input-label mapping, are: (1) the input examples, (2) the label examples and (3) the input-label format.
We then propose a series of variants of \demo\ that quantify the impact of different compositions of each component (Table~\ref{tab:abl-methods}).
We carefully design each variant to preserve the overall format of the \demo\ as much as possible.

\subsection{Method}

\vspace{.3em}
\noindent
\textbf{OOD \demo} include out-of-domain (OOD) text instead of the input examples from unlabeled training data. A set of $k$ sentences $\{x_{i,\mathrm{rand}}\}_{i=1}^k$ are randomly sampled from an external corpus,\footnote{
    We use CC-News~\citep{nagel2016cc} as an external corpus. We consider the length of the text during sampling, so that sampled sentences have similar length to the test input.
} and replace $x_1...x_k$ with unlabeled training data in the \demo. %Each sentence is paired with either a random label, a constant label or no labels, as we did with in-domain unlabeled data.
This variant removes the impact of conditioning on example inputs from the in-domain training data.

\vspace{.3em}
\noindent
\textbf{\Demo\ w/ constant labels} are composed with the constant text,  \texttt{answer}, as labels for all $k$ pairs.
%replaces all labels in the \demo\ to the constant text, \texttt{answer}.
Formally, a prediction is made via $\mathrm{argmax}_{y \in \mathcal{C}}P(y|x_1,\texttt{answer}...x_k,\texttt{answer},x)$.
This is to remove the impact of conditioning on the example labels since $\mathcal{C}$ is not used, while still using the input-label pairs as the {\em form} of the \demo.

\vspace{.3em}
\noindent
\textbf{\Demo\ with no labels} are composed with the input examples only, and labels are removed.
Specifically, a prediction is made via $\mathrm{argmax}_{y \in \mathcal{C}}P(y|x_1...x_k,x)$.
This removes the impact of using pairs as the form of the \demo, but still provides the example inputs.

\vspace{.3em}
Additional variants can be made by combining these three variants, e.g., using OOD inputs with constant labels or no labels. We present all possible variants in Table~\ref{tab:abl-methods}.
%summarizes all compositions as well as components in the \demo\ that are preserved in the variant.

\subsection{Results}\label{subsec:abl_result}
Figure~\ref{fig:main-results} reports model performance on 5 classification and 4 multi-choice datasets (same as datasets in Section~\ref{subsec:abl_accuracy}). Since we already observed that removing the groundtruth input-label mapping (\goldbox$\xrightarrow{}$\randombox) does not drop the performance much, we focus on the effect of other three components.

\vspace{-.1em}
\paragraph{Impact of the example inputs is significant.} Using OOD inputs instead of inputs from the training data significantly drops the performance.\footnote{With an exception of Direct MetaICL, which we explain in the later of the section. \ari{I would just make this part of the running text}} In particular, in Direct GPT-J, using OOD inputs with random labels is worse than no-\demo.
This is likely because the example inputs from the training data makes the distributions of inputs closer to the test input,
and this makes in-context learning closer to language modeling since the LM was trained to be conditioned on the in-distribution text.
Nonetheless, it is worth noting that conditioning on the example inputs is not the {\em only} factor that leads to performance gains: the \demo\ with the example inputs and no labels does not substantially improve the performance over no-\demo. \ari{It would be worth pointing gout that this changes the format, and thus the ``trigger'' for producing an answer. Also maybe we want color-coded blocks to indicate the only-inputs to no-demos contrast?}

\vspace{-.1em}
\paragraph{Impact of the example labels (\randombox$\xrightarrow{}$\answerbox) is as significant.} Using constant labels or no labels instead of random labels significantly drops the performance across all models.
We hypothesize that this is because the label space specified by the example labels leads to performance gains.
%\footnote{For instance, in classification, Direct MetaICL assigns over 94\% of its probability mass to the set of labels given the \demo\ with either gold labels or random labels.}
This is true even for multi-choice tasks where there is no fixed set of labels---it is likely that multi-choice tasks still do have a particular distribution of the choices (e.g., objects like ``Bolts'' or ``Screws'' in the OpenBookQA dataset) so that the model exploits it.

\vspace{-.1em}
\paragraph{The form of the pairs (\answerbox$\xrightarrow{}$\nolabelbox) is important in classification for channel.}
Using constant labels outperforms using no labels by 7--11\% absolute, and no-\demo\ by 10--14\% absolute.
This is interesting since simply keeping a specific format with pairs makes substantial difference in performance, and significantly outperforms no-\demo\ when combined with the inputs from the training data.
Note that this is not true in direct models---this suggests that channel models outperforming direct models in classification might be because channel models exploit the format of the pairs better than direct models. In multi-choice tasks, using constant labels and  no labels are marginally different, indicating that keeping the ``pairs'' matters less. 
This is likely because the distinction between the input and the label is often less obvious in multi-choice tasks (e.g. in sentence completion) because the labels change for each question and are not directly inferrable from \demo.

\vspace{-.1em} 
\paragraph{MetaICL learns to ignore information unsupervised LMs can't make use of.}
We additionally examine the results of MetaICL in order to identify the effect of meta-training with an in-context learning objective.
Our findings suggest that \textbf{meta-training captures whichever component that is easier to leverage, and encourages the model to make more use it}.
We find that it typically strengthens the impact of components that are more significant and easier to capture, and weakens the impact of components that are less significant (e.g., input-label mapping)
For instance, gains in Direct MetaICL are mostly from the example labels and conditioning on the text (even if it is not from the training data).\footnote{
    We hypothesize the direct model somehow found it easier to exploit ``conditioning on (either in-domain or out-of-domain) text'' rather than ``conditioning on in-domain text'' so that the sources of the inputs matter little.
}
Gains from Channel MetaICL are mostly from the example labels and the form of the pairs. We see even less impact of the input-label mapping in these meta-trained models, likely because learning to learn the groundtruth input-label mapping is much harder, thus models are trained toward the direction of ignoring it.

\vspace{.4em}
To summarize, except for the input-label mapping, all of the example inputs, the example labels and the form the input-label pairs are overall important for the task performance: \textbf{all models require at least two out of three to achieve meaningful improvements over no-demonstration}.
Although how much each component exactly matters varies across different types of models, results of the best models for each task indicate that the gains mostly come from both the example inputs and outputs, and also from the form of the input-label pairs in the case of classification.


==> sections/06-silver-zero-shot.tex <==
\begin{algorithm}[t]
\captionsetup{font=10pt} 
\caption{Methods with the silver demonstration.}\label{alg:silver}
\begin{algorithmic}[1] \footnotesize
\State {\protect\color{gitgreen}  {\textit{// $x$: test input, $\mathcal{X}$: a set of $k$ inputs}}} 
%
%\State {\protect\color{gitgreen}  {\textit{// Use No-demonstration to unlabeled data}} }
\State {\protect\color{gitgreen}  {\textit{// }} }
\Procedure{\textsc{SilverDemons}}{$x, \mathcal{X}$}
\State $D \gets [ ]$ {\protect\color{gitgreen}  {\textit{// demonstration to be formed}}} 
\For{$x_i \in \mathcal{X}$}
    \State {\protect\color{gitgreen}  {\textit{//  Use No-demonstration}} }
    \State $\tilde{y}_i \gets \mathrm{argmax}_{y \in \mathcal{C}}P(y|x_i)$ 
    \State $D\mathrm{.append}((x_i, \tilde{y}_i))$
\EndFor
\State \Return $\mathrm{argmax}_{y \in \mathcal{C}}P(y|D,x)$
\EndProcedure
%
%\State {\protect\color{gitgreen}  {\textit{// Use its own silver demonstration to unlabeled data}} }
\State {\protect\color{gitgreen}  {\textit{// }} }
\Procedure{\textsc{IterSilverDemons}}{$x, \mathcal{X}$}
\State $D \gets [ ]$ {\protect\color{gitgreen}  {\textit{// demonstration to be formed}}} 
\For{$x_i \in \mathcal{X}$}
    \State {\protect\color{gitgreen}  {\textit{//  Use its own silver demonstration}} }
    \State $\tilde{y}_i \gets \mathrm{argmax}_{y \in \mathcal{C}}P(y|D,x_i)$
    \State $D\mathrm{.append}((x_i, \tilde{y}_i))$
\EndFor
\State \Return $\mathrm{argmax}_{y \in \mathcal{C}}P(y|D,x)$
\EndProcedure
\end{algorithmic}
\end{algorithm}

Motivated by observations from previous sections, this section aims to build a better zero-shot method by leveraging the demonstration without labeled training data.

\subsection{Method}
We start from \textbf{Random demonstration} in Section~\ref{subsec:main}, and additionally introduce
\textsc{Silver} demonstration and \textsc{IterSilver} demonstration. All methods form the silver demonstration by using the LM to make a prediction on in-domain unlabeled data $x_i \in \mathcal{X}$ ($1 \leq i \leq k$), and then use the silver demonstration to make a prediction on the test input.

\begin{table}[t]
    \centering \footnotesize
    \setlength{\tabcolsep}{0.3em}
    \begin{tabular}{lccc}
        \toprule
            Method & Demons & Labeled & Unlabeled  \\
        \midrule
            No-demons & \xmark & \xmark & \xmark \\
            Gold demons & \cmark & \cmark & \cmark \\
        \midrule
            Random demons & \cmark & \xmark & \cmark \\
            \textsc{Silver} demons & \cmark & \xmark & \cmark \\
            \textsc{IterSilver} demons & \cmark & \xmark & \cmark \\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{Summary of our methods and baselines in Section~\ref{sec:silver}.
    {\em Demons} indicates whether the demonstration is used; {\em labeled} indicates whether in-domain labeled data is used; {\em unlabeled} indicates whether in-domain unlabeled data is used.
    Note that `No-demons' and `Gold demons' are typical zero-shot and in-context learning methods, respectively.
    }\label{tab:silver-methods}
\end{table}

\begin{figure}
\centering \footnotesize
\textcolor{white}{\rule{7cm}{4cm}}
\caption{
    Results of methods that do not use labeled data.}\label{fig:silver-result}
\end{figure}


\vspace{.3em}
\noindent
\textbf{Random demonstration} makes a random prediction for each $x_i \in \mathcal{X}$, as described in Section~\ref{subsec:main}.

\vspace{.3em}
\noindent
\textbf{\textsc{Silver} demonstration} (the first in Algorithm~\ref{alg:silver}) makes a prediction for each $x_i \in \mathcal{X}$ by using the no-demonstration method: $\tilde{y}_i = \mathrm{argmax}_{y \in \mathcal{C}}P(y|x_i)$. Then, $(x_1, \tilde{y}_1)...(x_k, \tilde{y}_k)$ is used as a silver demonstration that is fed when making a prediction to the test input.

\vspace{.3em}
\noindent
\textbf{\textsc{IterSilver} demonstraction} (the second in Algorithm~\ref{alg:silver}) sequentially makes a prediction for $x_1...x_k$. It first uses the no-demonstration method for $x_1$, and then uses $(x_1, \tilde{y}_1)...(x_{i-1}, \tilde{y}_{i-1})$ as the demonstration to make a prediction for $x_i$ ($i \geq 2$). Intuitively, this will lead to more accurate labels than \textsc{SilverDemons} for $i \geq 2$ given that using the demonstration is better than the no-demonstration method even if the demonstration is inaccurate.

\vspace{.3em}
We compare the above methods with (1) No-Demonstration, (2) Gold Demonstration, and (3) No-Demonstration with engineered templates. The last model is the only one in this paper that uses engineered templates instead of minimal templates, which we compare against to show that our methods outperform a competitive previous, engineered zero-shot method, despite not relying on such engineering.
%\footnote{As detailed in Appendix~\ref{app:exp-details}, engineered templates typically improve the no-demonstration method only; we were unable to find templates that consistently improve the demonstration method.}
More details are provided in Appendix~\ref{app:exp-details}.

\subsection{Results}
We experiment with the best ICL-trained model and the best non-ICL-trained model under 13B: Channel MetaICL and Channel GPT-J for classification tasks, and Channel MetaICL and Direct GPT-J for multi-choice tasks. We evaluate on 4 classification datasets and 4 multi-choice datasets as in Section~\ref{sec:abl}.

Results are reported in Figure~\ref{fig:silver-result}.
